Lookahead Acquisition Functions for Finite-Horizon Time-Dependent Bayesian Optimization and Application to Quantum Optimal Control

We propose a novel Bayesian method to solve the maximization of a time-dependent expensive-to-evaluate stochastic oracle. We are interested in the decision that maximizes the oracle at a finite time horizon, given a limited budget of noisy evaluations of the oracle that can be performed before the horizon. Our recursive two-step lookahead acquisition function for Bayesian optimization makes nonmyopic decisions at every stage by maximizing the expected utility at the specified time horizon. Specifically, we propose a generalized two-step lookahead framework with a customizable \emph{value} function that allows users to define the utility. We illustrate how lookahead versions of classic acquisition functions such as the expected improvement, probability of improvement, and upper confidence bound can be obtained with this framework. We demonstrate the utility of our proposed approach on several carefully constructed synthetic cases and a real-world quantum optimal control problem.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

\newcommand{\defeq}{:=}
\newcommand{\PI}{\textrm{PI}}
\newcommand{\EI}{\textrm{EI}}
\newcommand{\UCB}{\textrm{UCB}}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Time-dependent Bayesian Optimization}{Renganathan, Larson, and Wild}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Lookahead Acquisition Functions for Finite-Horizon Time-Dependent \\ Bayesian Optimization and Application to Quantum Optimal Control\thanks{\funding{U.S.\ Department of Energy, Office of Science, Advanced Scientific Computing Research, %Quantum Algorithm Teams Program 
QAT4ChemSci, FAR-QC, and AIDE-QC projects
under Contract DE-AC02-06CH11357}}}

% Authors: full names plus addresses.
\author{S. Ashwin Renganathan{\thanks{Mathematics \& Computer Science Division, Argonne National Laboratory, Lemont, IL 
  (\email{srenganathan@anl.gov}, \email{jmlarson@anl.gov}, \email{wild@anl.gov}).}}
  \and
  Jeffrey Larson\footnotemark[2]
  \and 
    %SW ORCID: 0000-0002-6099-2772
  Stefan M.\ Wild\footnotemark[2]
  }

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

